Who Taught the Robot That? Removing One User's Corrections from a Robot Policy That Learns Online

A robot that keeps learning after deployment is corrected by several people in turn, and one of them may later ask to be removed. We show that whether the robot can forget that person depends on how people correct it. The goal of removal is the robot that would exist if the person had never been there, which we compute exactly in two simulated tasks with scripted users. When users correct the robot by taking over control, an ordered log of training updates is enough: retraining on the remaining sessions in their original order gives a robot as close to the goal as training noise allows. Deleting the person's data and retraining in one pass does not, even when the other users' corrections do not depend on the removed person, because it loses the order of training. When users only nudge the robot's action, the other users' corrections carry the removed person's influence, and no method we tested recovers the goal robot. Continuing to train without the person removes most of their habits, but not what their data in the training buffer keep alive. The log can identify one clearly harmful user, but not rank users by influence better than counting their corrections.

==> rugh.tex <==
Hi all, sharing a proposal for two simulation benchmarks for VLAs/robot foundation models (doc attached). It covers a survey of current benchmarks (LIBERO, SimplerEnv, RoboTwin, BEHAVIOR, RoboArena, etc.), how models are actually evaluated (mostly fine-tuned on each benchmark’s own data, so published numbers are rarely comparable), the gaps, and detailed designs for both:

RAD-Bench (Robustness, Adaptation, Disturbance): how policies degrade, recover and adapt under graded physical disturbances (external forces, mass/friction changes, actuator gain, action delay, mid-episode dynamics changes). It uses a fixed fine-tuning budget, and every severity level is calibrated so an expert can still solve the task.
OccluProp-Bench: whether policies keep acting correctly when the target becomes hidden during the task (object permanence), and which sensor they trust when camera and proprioception disagree.

Both run in ManiSkill3 on one shared harness. A small real-robot study is planned only to check that simulation rankings transfer.

Possible target: RSS 2027’s new two-stage track. Stage 1 (Dec 4) reviews the problem and methodology and allows preliminary experiments; full results are due April 16. OccluProp-Bench could follow at IROS 2027 (Mar 1).

Would love feedback, especially on: which models we must include, available GPU resources, whether to do one paper or two, and anyone interested in contributing. Comments in the doc work too.
